QUIJOTE scientific results - XII. Characterization of the polarized synchrotron emission at the power spectrum level in the QUIJOTE-MFI wide survey

We present an analysis of the polarized synchrotron emission at the power-spectrum level in the multipole range $30 < \ell < 130$, using the recent QUIJOTE-MFI wide survey (10-20GHz) in combination with Planck and WMAP data. The EE and BB power spectra are well described by a simple power-law model, with no evidence for the need of additional parameters. The best-fit slopes are $\alpha_{EE} = -3.24 \pm 0.12$ and $\alpha_{BB} = -3.81 \pm 0.34$ for $|b|>20^\circ$, hinting toward a steepening of the BB spectrum relative to EE at the $\sim 1.6\sigma$ level. The synchrotron frequency spectral indices are found to be $\beta_s^{EE} = -3.26 \pm 0.05$ and $\beta_s^{BB} = -3.25 \pm 0.10$ for the same cut, in agreement with earlier real-space analyses. We find no evidence for spatial variations of $\beta_s$ across different Galactic latitude cuts, within current uncertainties. The synchrotron BB/EE power ratio is approximately 0.2 over the considered multipole range, lower than typical values for thermal dust, and consistent with previous measurements. We also measure a dust-synchrotron spatial correlation in the range 0.1-0.25 over $30 < \ell < 130$. Using these results, we estimate the level of synchrotron contamination in future CMB B-mode measurements, finding an average power in the considered sky masks equivalent to $r \sim 0.003$ at 90GHz and $r \sim 0.0002$ at 150GHz for the relevant angular scales.

==> figs/tabfit.tex <==
\begin{table}
\centering
\caption{Results of the power law fit to the synchrotron $EE$ and $BB$ power spectra. The corr. line indicates the linear correlation between the errors on the two parameters $A_s$ and $\alpha$.}\label{tab:specfit}
\begin{tabular}{ccccc}
  \hline
     &  & $\pm 10^\circ$     &  $\pm 15^\circ$    & $\pm 20^\circ$\\
  \hline
  \hline
     & $A_s \, (10^{-3}\mu K^2)$ & $ 9.63 \pm 0.43 $ & $ 8.09 \pm 0.42 $ & $ 7.09 \pm 0.43 $ \\
  EE & $\alpha $                 & $ -3.09 \pm 0.09 $ & $ -3.13 \pm 0.1 $ & $ -3.24 \pm 0.12 $ \\
     & corr.                     &  0.54  &   0.58   &  0.62  \\
  \vspace{1mm} \vspace{-3.5mm} \\
\hline
  \vspace{1mm} \vspace{-3.5mm} \\
     & $A_s \, (10^{-3}\mu K^2)$ & $ 1.52 \pm 0.22 $ & $ 1.06 \pm 0.2 $ & $ 0.93 \pm 0.22 $ \\
  BB & $\alpha $                 & $ -3.54 \pm 0.22 $ & $ -3.84 \pm 0.28 $ & $ -3.81 \pm 0.34 $ \\
     & corr.                     &  0.86  &   0.89   &  0.9  \\
   \hline
\end{tabular}
\end{table}

==> figs/tabfit_WM+Pl+QJ.tex <==
\begin{table}
  \centering
  \caption{Results of the power law fit to the synchrotron $EE$ and $BB$ power spectra for the  WM+Pl+QJ  set. The corr. line indicates the linear correlation between the errors on the two parameters $A_s$ and $\alpha$.}\label{tab:specfit}
  \begin{tabular}{ccccc}
    \hline
       &  & $\pm 10^\circ$     &  $\pm 15^\circ$    & $\pm 20^\circ$\\
    \hline
    \hline
       & $A_s \, (10^{-3}\mu K^2)$ & $ 9.63 \pm 0.43 $ & $ 8.09 \pm 0.42 $ & $ 7.09 \pm 0.43 $ \\
    EE & $\alpha $                 & $ -3.09 \pm 0.09 $ & $ -3.13 \pm 0.1 $ & $ -3.24 \pm 0.12 $ \\
       & corr.                     &  0.54  &   0.58   &  0.62  \\
    \vspace{1mm} \vspace{-3.5mm} \\
  \hline
    \vspace{1mm} \vspace{-3.5mm} \\
       & $A_s \, (10^{-3}\mu K^2)$ & $ 1.52 \pm 0.22 $ & $ 1.06 \pm 0.2 $ & $ 0.93 \pm 0.22 $ \\
    BB & $\alpha $                 & $ -3.54 \pm 0.22 $ & $ -3.84 \pm 0.28 $ & $ -3.81 \pm 0.34 $ \\
       & corr.                     &  0.86  &   0.89   &  0.9  \\
     \hline
  \end{tabular}
  \end{table}

==> figs/tabfit_WM+Pl.tex <==
\begin{table}
  \centering
  \caption{Results of the power law fit to the synchrotron $EE$ and $BB$ power spectra for the  WM+Pl  set. The corr. line indicates the linear correlation between the errors on the two parameters $A_s$ and $\alpha$.}\label{tab:specfit}
  \begin{tabular}{ccccc}
    \hline
       &  & $\pm 10^\circ$     &  $\pm 15^\circ$    & $\pm 20^\circ$\\
    \hline
    \hline
       & $A_s \, (10^{-3}\mu K^2)$ & $ 9.26 \pm 0.59 $ & $ 7.62 \pm 0.59 $ & $ 6.81 \pm 0.61 $ \\
    EE & $\alpha $                 & $ -3.1 \pm 0.12 $ & $ -3.17 \pm 0.14 $ & $ -3.26 \pm 0.16 $ \\
       & corr.                     &  0.69  &   0.74   &  0.76  \\
    \vspace{1mm} \vspace{-3.5mm} \\
  \hline
    \vspace{1mm} \vspace{-3.5mm} \\
       & $A_s \, (10^{-3}\mu K^2)$ & $ 2.07 \pm 0.36 $ & $ 1.47 \pm 0.36 $ & $ 1.39 \pm 0.39 $ \\
    BB & $\alpha $                 & $ -2.96 \pm 0.28 $ & $ -3.29 \pm 0.37 $ & $ -3.18 \pm 0.43 $ \\
       & corr.                     &  0.86  &   0.9   &  0.89  \\
     \hline
  \end{tabular}
  \end{table}

==> figs/table_betas.tex <==
\begin{table}
\centering
\caption{Fitted synchrotron spectral index $\beta_{\rm s}$ values, for the EE and BB power spectra, and for the main data sets. The values are plotted in Fig.~\ref{fig:betas}.}
\begin{tabular}{ccccc}
\hline
& & $\pm 10^\circ$     &  $\pm 15^\circ$    & $\pm 20^\circ$ \\
\hline
\hline
EE  &  WM+Pl & 
$ -3 \pm  0.09 $&
$ -3.05 \pm  0.11 $&
$ -3.12 \pm  0.12 $\\
EE  &  WM+Pl+QJ & 
$ -3.22 \pm  0.03 $&
$ -3.24 \pm  0.03 $&
$ -3.26 \pm  0.03 $\\
\hline
BB  &  WM+Pl & 
$ -2.83 \pm  0.2 $&
$ -3.01 \pm  0.25 $&
$ -3.01 \pm  0.3 $\\
BB  &  WM+Pl+QJ & 
$ -3.33 \pm  0.07 $&
$ -3.34 \pm  0.08 $&
$ -3.25 \pm  0.1 $\\
\hline
\end{tabular}
\label{tab:betas}
\end{table}

